Ambisonics Networks -- The Effect Of Radial Functions Regularization

Ambisonics, a popular format of spatial audio, is the spherical harmonic (SH) representation of the plane wave density function of a sound field. Many algorithms operate in the SH domain and utilize the Ambisonics as their input signal. The process of encoding Ambisonics from a spherical microphone array involves dividing by the radial functions, which may amplify noise at low frequencies. This can be overcome by regularization, with the downside of introducing errors to the Ambisonics encoding. This paper aims to investigate the impact of different ways of regularization on Deep Neural Network (DNN) training and performance. Ideally, these networks should be robust to the way of regularization. Simulated data of a single speaker in a room and experimental data from the LOCATA challenge were used to evaluate this robustness on an example algorithm of speaker localization based on the direct-path dominance (DPD) test. Results show that performance may be sensitive to the way of regularization, and an informed approach is proposed and investigated, highlighting the importance of regularization information.

==> table.tex <==
% \usepackage{array,makecell}\

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|p{2cm}|p{2.5cm}|p{2.5cm}|}
  \hline
  \textbf{Parameters} & \textbf{Train set} & \textbf{Test set} \\
  \hline
  \# of speech signals. & 7 & 10
  \\
  \hline
  Room Sizes [\(m \times m \times m \)] & 
  \( 3 \times 4 \times 2\),
  \( 4 \times 6 \times 5\),
  \( 10 \times 6 \times 8\).
  & 
  \( 5 \times 3 \times 4\),
  \( 7 \times 6 \times 3\).
  \\
  \hline
  Array center &  \multicolumn{2}{|p{5cm}|}{Randomly chosen for each room, 0.5m at least from walls.}  \\
  \hline
  T60 [sec] & 0.25, 0.5, 0.75, 1. & 0.33, 0.66, 0.99, 1.5. \\
  \hline
  SNR [dB] & 20, 30, 50.  & 10, 5. \\
  \hline
  Source array distance & \multicolumn{2}{|p{5cm}|}{
  \(0.5r_d, r_d, 2r_d, 3r_d\). \(r_d\) is the critical distance. depend on the scenario, value was reduced to keep source in the room.}
  \\
  \hline
  \(\lambda\)  values.  & 0.001. & 0.001, 0.01, 0.1, 1. \\
  \hline
\end{tabular}
\end{adjustbox}
